Model-based construction of Open Non-uniform Cylindrical Algebraic Decompositions

In this paper we introduce the notion of an Open Non-uniform Cylindrical Algebraic Decomposition (NuCAD), and present an efficient model-based algorithm for constructing an Open NuCAD from an input formula. A NuCAD is a generalization of Cylindrical Algebraic Decomposition (CAD) as defined by Collins in his seminal work from the early 1970s, and as extended in concepts like Hong's partial CAD. A NuCAD, like a CAD, is a decomposition of n-dimensional real space into cylindrical cells. But unlike a CAD, the cells in a NuCAD need not be arranged cylindrically. It is in this sense that NuCADs are not uniformly cylindrical. However, NuCADs--- like CADs --- carry a tree-like structure that relates different cells. It is a very different tree but, as with the CAD tree structure, it allows some operations to be performed efficiently, for example locating the containing cell for an arbitrary input point.

==> ex1/README <==
Initial try:

F := [ 2 y z - x^2 < 0 /\ x^2 + y^2 + z^2 - 1 < 0 ]

[]
(x,y,z)
3
[
2 y z - x^2 < 0 /\ x^2 + y^2 + z^2 - 1 < 0
].

* C0: R^3,{},"",(1/3,1/3,1/3)

* Split(C0)
  F false @ (1/3,1/3,1/3).
  Choose 2 y z - x^2, which is > 0 at alpha
(def CX (new-ocbuilder '(x y z) '(1/3 1/3 1/3) '([2 y z - x^2])))
C1: 3X [ z > _root_1 2 y z - x^2  /\ y > _root_1 y ]  (1/3 1/3 1/3)
C2: 2L [ y < 0 ] (1/3,-1/3,1/3)
C3: 3L [ z < _root_1 2 y z - x^2  /\ y > 0 ] (1/3 1/3 -1/3)

* Split(C2)
  F true @ (1/3,-1/3,1/3)
  Choose 2 y z - x^2 , x^2 + y^2 + z^2 - 1
(def CX (new-ocbuilder '(x y z) '(1/3 -1/3 1/3) '([2 y z - x^2] [x^2 + y^2 + z^2 - 1] [y])))
C4: 2L3X [ z > _root_1 2 y z - x^2 /\ z < _root_2 z^2 + y^2 + x^2 - 1  /\ y > _root_1 2 y^2 + 2 y + x^2 /\ y < _root_2 2 y^2 + 2 y + x^2  /\ x > _root_1 x /\ x < _root_2 2 x^2 - 1 ]  (1/3 -1/3 1/3)
C5: 2L1L [ x < 0 /\ y < 0 ] (-1/3 -1/3 1/3)
C6: 2L1U [ x > _root_2 2 x^2 - 1 /\ y < 0 ] (4/3 -1/3 1/3)
C7: 2L2L [ y < _root_1 2 y^2 + 2 y + x^2 /\ x > _root_1 x /\ x < _root_2 2 x^2 - 1 ] (1/3 -2 1/3)
C8: 2L2U [  y > _root_2 2 y^2 + 2 y + x^2 /\ y < 0  /\ x > _root_1 x /\ x < _root_2 2 x^2 - 1 ] (5/16 -1/64 1/3)
C9: 2L3L [ z < _root_1 2 y z - x^2  /\ y > _root_1 2 y^2 + 2 y + x^2 /\ y < _root_2 2 y^2 + 2 y + x^2  /\ x > _root_1 x /\ x < _root_2 2 x^2 - 1 ] (1/3 -1/3 -2)
C10: 2L3U [ z > _root_2 z^2 + y^2 + x^2 - 1  /\ y > _root_1 2 y^2 + 2 y + x^2 /\ y < _root_2 2 y^2 + 2 y + x^2  /\ x > _root_1 x /\ x < _root_2 2 x^2 - 1 ]  (1/3 -1/3 2)


* Split(C3)
  F true @ (1/3 1/3 -1/3)
  Choose   x^2 + y^2 + z^2 - 1
  (def CX (new-ocbuilder '(x y z) '(1/3 1/3 -1/3) '([2 y z - x^2] [x^2 + y^2 + z^2 - 1] [y])))

* Split(C10)
(def CX (new-ocbuilder '(x y z) '(1/3 -1/3 2) '([ z^2 + y^2 + x^2 - 1 ] [ 2 y^2 + 2 y + x^2 ] [ x ] [ 2 x^2 - 1 ])))
No split.  Already TI.

* Split(C7)
  F false @ (1/3 -2 1/3)
  Choose x^2 + y^2 + z^2 - 1
  (def CX (new-ocbuilder '(x y z) '(1/3 -2 1/3) '([x^2 + y^2 + z^2 - 1] [2 y^2 + 2 y + x^2] [x] [2 x^2 - 1])))
C11: 2L2L3X [ y < _root_1 y^2 + x^2 - 1  /\ x > _root_1 x /\ x < _root_2 2 x^2 - 1 ] (1/3 -2 1/3)


Final:
C0: R^3,{},"",(1/3,1/3,1/3)
C1: [ z > _root_1 2 y z - x^2  /\ y > 0 ] 3X (1/3,1/3,1/3)
    ( y:alg 2 y z - x^2:alg )
C3: [ z < _root_1 2 y z - x^2  /\ y > 0 ] 3L (1/3 1/3 -1/3)

==> ex2/CADout <==
[]
(x,y)
2
[ y > (x + 1/4)^2 /\ x^2 + y^2 - 1 > 0 ].
go
go
go
d-2d-cad E -2 2 -1.25 2.75 600 600 0.5
n
200
i
ex2CAD.eps
1
1

